TiBGL: Template-induced Brain Graph Learning for Functional Neuroimaging Analysis

In recent years, functional magnetic resonance imaging has emerged as a powerful tool for investigating the human brain's functional connectivity networks. Related studies demonstrate that functional connectivity networks in the human brain can help to improve the efficiency of diagnosing neurological disorders. However, there still exist two challenges that limit the progress of functional neuroimaging. Firstly, there exists an abundance of noise and redundant information in functional connectivity data, resulting in poor performance. Secondly, existing brain network models have tended to prioritize either classification performance or the interpretation of neuroscience findings behind the learned models. To deal with these challenges, this paper proposes a novel brain graph learning framework called Template-induced Brain Graph Learning (TiBGL), which has both discriminative and interpretable abilities. Motivated by the related medical findings on functional connectivites, TiBGL proposes template-induced brain graph learning to extract template brain graphs for all groups. The template graph can be regarded as an augmentation process on brain networks that removes noise information and highlights important connectivity patterns. To simultaneously support the tasks of discrimination and interpretation, TiBGL further develops template-induced convolutional neural network and template-induced brain interpretation analysis. Especially, the former fuses rich information from brain graphs and template brain graphs for brain disorder tasks, and the latter can provide insightful connectivity patterns related to brain disorders based on template brain graphs. Experimental results on three real-world datasets show that the proposed TiBGL can achieve superior performance compared with nine state-of-the-art methods and keep coherent with neuroscience findings in recent literatures.

==> Specific_implement.tex <==
\section{Specific implement}\label{implement}
In this section, we choose two graph embedding methods, consisting of LE \cite{belkin2003laplacian} and LLE \cite{roweis2000nonlinear}, to provide a typical implement for our proposed framework, named GCMF-LLE.

\subsection{The Construction Process of GCMF-LLE}
LLE lies on the manifold structure of the samples space to preserve the relationships among samples. Based on the assumption that each sample and its neighbors to lie on or close to a locally linear patch of the manifold, then we obtain the weights matrix $\bm{S}^v \in \mathbb{R}^{N \times N}$ by minimizing the following reconstruction error:
\begin{equation}\label{solve_weights}
    %Error \left( \bm{S}^v \right){=}
    {\sum\limits_{i = 1}^N {\| {\bm{X_i^v} - \sum\limits_{j \in \mathop{N}\{i\}} {{\bm{S}_{ij}^v}{\bm{X}_j^v}} } \|_2 ^2}}
\end{equation}
where $\mathop{N}\{i\}$ denotes the neighbors of the $i$th sample $\bm{X}_i^v$. By solving the above equation, we could obtain graph structure $\bm{S}^v$ to reflect intrinsic properties of the samples space. We expect their characterization of local geometry in the original space to be equally valid for local patches on the manifold. Each original sample $\bm{X}_i^v$ is mapped to a new $d^v$-dimensional coordinate. %This is done by choosing  to minimize the following embedding cost function:
%\begin{equation}
%    Error \left( \bm{U}^v \right){=}{\sum\limits_{i = 1}^N {\| {{\bm{U}_i^v} - %\sum\limits_{j \in \mathop{N}\{i\}} {{\bm{S}_{ij}^v}{\bm{U}_j^v}} } \|_2 ^2}}
%\end{equation}
Additionally, we constrain the learned representations $\bm{U}_i^v, 1 \le i \le N$ to have unit covariance. With simple algebraic formulation, the above cost problem can be further transformed as follows:
\begin{equation}\label{lle}
\begin{array}{l}
\mathop {\min }\limits_{\bm{U}^v} \hspace{0.5em} tr(\bm{U}^{v}\bm{{({I-S^v})}^T(I-S^v)}\bm{U^{v^T}})\\
\hspace{0.5em}s.t.\hspace{1em}\bm{U}^{v}\bm{U}^{v^T} = \bm{I}
\end{array}
\end{equation}
Hereto, we determine that $\mathcal{F}(\bm{U}^v)$ and $\mathcal{\bm{C}}^v$ are responding to $tr(\bm{U}^{v}\bm{{({I-S^v})}^T(I-S^v)}\bm{U^{v^T}})$ and $\bm{U}^{v}\bm{U}^{v^T} = \bm{I}_N$ respectively.

LE aims at preserving the local neighborhood structure on the data manifold, which constructs the weight matrix that describes the relationships among the samples. Specifically, the similarity matrix $\bm{G}_{\ast}$ is to denote the weight coefficients, which could choose the common kernel function as our similarity measure, such as linear kernel, polynomial kernel, Gaussian kernel and etc. Combining this with the graph consensus term in between the $v$ view and $w$th view, we could define $\bm{L}^w$ as follows:
\begin{equation}
\begin{split}
& \bm{L}^w = \bm{D}^w-\bm{G}_{\ast}^w\\
\end{split}
\end{equation}
where $\bm{D}^w$ denotes a diagonal matrix and ${\bm{D}_{ii}^w}=\sum\limits_j {{{\bm{G}_{\ast}}^w_{ij}}}$. By rewriting the normalized matrix $\bm{L}^w$, we could get $\bm{L}^w=\bm{I}_N - {\bm{D}^w}^{ - 1/2}\bm{G}_{\ast}^w{\bm{D}^w}^{ - 1/2}$. Therefore, we can obtain the following graph consensus term between two views:
\begin{equation}
\begin{split}
& Reg(\bm{U}^v, \bm{G}_\ast^w) = tr\left( \bm{U}^v (\bm{I}_N - {\bm{D}^w}^{ - 1/2}\bm{G}_{\ast}{\bm{D}^w}^{ - 1/2}) {\bm{U}^v}^T \right) \\
\end{split}
\end{equation}

According to the above construction of single-view graph loss function and graph consensus term between views, we have specified each term in objective function in and its constraint terms. In this way, we could extend single-view based LLE into multi-view setting, named Multi-view Locality Linear Embedding (GCMF-LLE). Accordingly, the whole objective function for GCMF-LLE can be formulated as follows:
\begin{equation}
\begin{split}
& \mathop {\min}\mathcal{\bm{O}}\left( \bm{U}^1, \bm{U}^2, \ldots, \bm{U}^M \right) = \\
& \sum_{v=1}^M tr(\bm{U}^{v}\bm{{({I-S^v})}^T(I-S^v)} \bm{U^{v^T}}) + \lambda_{R} \sum_{v=1}^M \bm{\Omega}(\bm{U}^v)\\
& +  \lambda_{C} \sum_{v \neq w} {tr\left( \bm{U}^v (\bm{I}_N - {\bm{D}^w}^{ - 1/2}\bm{G}_{\ast}^w{\bm{D}^w}^{ - 1/2}) {\bm{U}^v}^T \right)}\\
&\hspace{0.5em}s.t.\hspace{1em}\bm{U}^{v}\bm{U}^{v^T} = \bm{I}, 1 \le v \le M \\
\end{split}
\end{equation}
Because the constraint terms normalize the scale of $\{\bm{U}^1, \bm{U}^2, \ldots, \bm{U}^M\}$, the smooth regularized term $\bm{\Omega}(\bm{U}^v)$ could be neglected in the objective function of GCMF-LLE. That is, the above equation could be reduced as follows:
\begin{equation} \label{total_loss_lle}
\begin{split}
& \mathop {\min}\mathcal{\bm{O}}\left( \bm{U}^1, \bm{U}^2, \ldots, \bm{U}^M \right) = \\
& \sum_{v=1}^M tr(\bm{U}^{v}\bm{{({I-S^v})}^T(I-S^v)} \bm{U^{v^T}}) \\
& +  \lambda_{C} \sum_{v \neq w} {tr\left( \bm{U}^v (\bm{I}_N - {\bm{D}^w}^{ - 1/2}\bm{G}_{\ast}^w{\bm{D}^w}^{ - 1/2}) {\bm{U}^v}^T \right)}\\
&\hspace{0.5em}s.t.\hspace{1em}\bm{U}^{v}\bm{U}^{v^T} = \bm{I}, 1 \le v \le M \\
\end{split}
\end{equation}

\subsection{Optimization}
Referring to the optimization procedure for GCMLF, the Eq.(\ref{total_loss_lle}) could be approximately solved. When solving the $v$th view, with all views fixed but $\bm{U}^v$, we get the following optimization for the $v$th view:
\begin{equation}
\begin{split}
& \mathop {\min}\mathcal{\bm{O}}\left( \bm{U}^v \right) = tr\left(\bm{U}^{v}\bm{{({I-S^v})}^T(I-S^v)} \bm{U^{v^T}}\right) \\
& +  \lambda_{C} \sum_{1 \le v \neq w}^M {tr\left( \bm{U}^v (\bm{I}_N - {\bm{D}^w}^{ - 1/2}\bm{G}_{\ast}^w{\bm{D}^w}^{ - 1/2}) {\bm{U}^v}^T \right)}\\
&\hspace{0.5em}s.t.\hspace{1em}\bm{U}^{v}\bm{U}^{v^T} = \bm{I} \\
\end{split}
\end{equation}

Due to the attributes of the matrix trace, the above equation is equivalent to the following optimization problem:
\begin{equation}\label{lle_view}
\begin{split}
& \mathop {\min}\mathcal{\bm{O}}\left( \bm{U}^v \right) = tr(\bm{U}^{v} ( \bm{{({I-S^v})}^T(I-S^v)} + \\
& \lambda_{C} \sum_{1 \le v \neq w}^M { (\bm{I}_N - {\bm{D}^w}^{ - 1/2}\bm{G}_{\ast}^w{\bm{D}^w}^{ - 1/2}) }  \bm{U^{v^T}}) \\
&\hspace{0.5em}s.t.\hspace{1em}\bm{U}^{v}\bm{U}^{v^T} = \bm{I} \\
\end{split}
\end{equation}
Under the constraint condition $\bm{U}^{v}\bm{U}^{v^T} = \bm{I}$, the above equation could be efficiently solved by eigenvalue decomposition. In this way, we could solve all the variables $\{\bm{U}^v,\bm{G}_{\ast}^v, 1\le v \le M\}$ iteratively.
%and the whole procedure to solve GCMF-LLE is summarized in \textbf{Algorithm \ref{algo-2}}.

According to the convergence analysis for our framework in Section , it could be easily verified that he optimization procedure for GCMF-LLE will be converged within limited iteration steps. We also use many experiments to verify the convergence property of the proposed method. Fig. shows the relation between the objective values and iterations. As shown in Fig. , we can see that with the iterations increase, the objective function value of the proposed method decreases fast and reaches a stable point after a few iterations, while the classification accuracy increases dramatically during the first small number of iterations and then reaches the stable high level for these four benchmark databases. For example, for the Holidays dataset, the proposed method reaches the stable point in terms of the classification accuracy within about fifteen iterations. Both theoretical proof and experiments demonstrate that the proposed method can obtain the local optimum quickly and has good convergence property.


